A Free Group of Rotations of Rank 2

One of the key steps in the proof of the Banach-Tarski Theorem is the introduction of a free group of rotations. First, a free group of reduced words is generated where each element of the set is represented as an ACL2 list. Then we demonstrate that there is a one-to-one relation between the set of reduced words and a set of 3D rotations. In this paper we present a way to generate this set of reduced words and we prove group properties for this set. Then, we show a way to generate a set of 3D matrices using the set of reduced words. Finally we show a formalization of 3D rotations and prove that every element of the 3D matrices set is a rotation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{76}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.8}{10.4204/EPTCS.359.8}}

